Self-DC: When to Reason and When to Act? Self Divide-and-Conquer for Compositional Unknown Questions

Previous research has typically concentrated on leveraging the internal knowledge of Large Language Models (LLMs) to answer known questions (i.e., \textit{internal reasoning such as generate-then-read}). In contrast, for questions that fall outside their known scope, these models rely on external knowledge retrieval to provide accurate responses (i.e., \textit{external acting such as retrieve-then-read}). However, few previous works consider the \textit{compositional questions}, which consist of several known and unknown sub-questions, necessitating the dynamic combination of previous two methods (i.e., \textit{internal reasoning and external acting}) to achieve a better trade-off between effectiveness and efficiency. To this end, we introduce a \textbf{Self} \textbf{D}ivide-and-\textbf{C}onquer (\textit{\texttt{Self-DC}}) framework, accompanying with the first \textbf{C}ompositional \textbf{u}nknown \textbf{Q}uestion-\textbf{A}nswering dataset (CuQA). This framework enables LLMs to adaptively choose between using internal knowledge and retrieving external knowledge as needed, resulting in a better trade-off between effectiveness and efficiency. Experimental results on two datasets demonstrate that \textit{\texttt{Self-DC}} can achieve comparable or even better performance with much fewer external calls compared with several strong baselines.

==> tables/append_freshqa_1106.tex <==
\begin{table}[!t]
  \centering
  \begin{adjustbox}{max width=0.48\textwidth}
  \begin{tabular}{l|ccc}
    \toprule
        \multirow{2}{*}{\textbf{Methods}} \hspace{8mm} & \multicolumn{3}{c}{\textbf{FreshQA}}  \\
    \cline{2-4} & \hspace{2mm} EM \hspace{2mm} & \hspace{2mm} F1 \hspace{2mm} & \hspace{2mm} Acc$^\dagger$ \hspace{2mm} \\
    \hline
    \hline
    \multicolumn{4}{c}{\textbf{\textit{w/o retrieval}}} \\
    \hline
    \hline
    Direct & 21.3 & 21.5 & 36.5  \\
    CoT & 20.8 & 21.6 & 36.0  \\
    Few-shot-CoT$^*$ & 18.7 & 11.9 & 31.6  \\
    GenRead & 18.2 & 17.1 & 36.3  \\
    \hline
    \hline
    \multicolumn{4}{c}{\textbf{\textit{w/ retrieval}}} \\
    \hline
    \hline
    RR & 36.0 & \textbf{32.4} & \underline{61.8}  \\
    REFEED & 23.2 & 14.3 & 39.0\\
    IRCoT & \textbf{37.5} & 16.5 & \underline{60.3}  \\
    Self-Ask$^*$ & 11.5 & 14.8 & 29.8  \\
    ITER-RETGEN$^*$ & 25.7 & 13.3 & 37.5 \\
    \hline
    % ### before results
    \textit{\textbf{Self-DC}} (\textit{verb}) & 35.2 & 27.1 & 56.0  \\ 
    \textit{\textbf{Self-DC}} (\textit{prob}) & \underline{36.8} & \underline{31.4} & \textbf{62.0}\\
    
    % beta = 0.1
    % \textit{\textbf{Self-DC}} (\textit{verb}) & 34.4 & 26.4 & 54.8  \\ 
    % % alpha=0.9, retr = 1017
    % % \textit{\textbf{Self-DC}} (\textit{verb}) & 30.2 & 28.2 & 54.8 49.3 \\ 
    % % alpha=0.7, retr = 298
    % \textbf{Self-DC} (\textit{prob}) & \underline{36.0} & \underline{32.1} & 59.3\\ 
    % % alpha=0.9, retr = 579
    % % \textbf{Self-DC} (\textit{prob}) & 36.0 & 31.3 & 59.7\\ 
    % % alpha=0.9, retr = 580

    
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{The performance of baselines and SelfDC with the \texttt{1106}. The baseline$^*$ means it uses demonstrations. We \textbf{bold} the highest performance and \underline{underline} the second-highest performance.}
% To provide deeper insights of SelfDC, we intentionally refrain from selecting $\alpha, \beta$ to make SelfDC equivalent to GenRead or RR. However, we emphasize we retain the flexibility to choose values for  $\alpha, \beta$ and can always ensure SelfDC is at least as effective as GenRead or RR.
\label{tab:append_freshqa_1106}
\end{table}

==> tables/append_freshqa_instruct.tex <==
\begin{table}[!t]
  \centering
  \begin{adjustbox}{max width=0.5\textwidth}
  \begin{tabular}{l|ccc}
    \toprule
        \multirow{2}{*}{\textbf{Methods}} \hspace{8mm} & \multicolumn{3}{c}{\textbf{FreshQA}}  \\
    \cline{2-4} & \hspace{2mm} EM \hspace{2mm} & \hspace{2mm} F1 \hspace{2mm} & \hspace{2mm} Acc$^\dagger$ \hspace{2mm} \\
    \hline
    \hline
    \multicolumn{4}{c}{\textbf{\textit{w/o retrieval}}} \\
    \hline
    \hline
    Direct & 19.0 & 8.2 & 38.3  \\
    CoT & 17.8 & 7.5 & 38.3  \\
    Few-shot-CoT$^*$ & 23.3 & 13.4 & 42.0  \\
    GenRead  & 21.5 & 7.8 & 36.3   \\
    \hline
    \hline
    \multicolumn{4}{c}{\textbf{\textit{w/ retrieval}}} \\
    \hline
    \hline
    RR & \textbf{33.0} & 12.1 & \underline{53.8}   \\
    REFEED & 19.2 & 10.1 & 35.7  \\
    IRCoT  & \underline{32.8} & \textbf{21.2} & \textbf{56.5}  \\
    Self-Ask$^*$ & 13.8 & 16.2 & 36.7 \\
    ITER-RETGEN$^*$ & 14.5 & 16.0 & 43.8  \\
    \hline
    % ### before
    % \textbf{Self-DC} (\textit{verb}) & 24.9 & 10.9 & 40.4 \\
    
    % beta = 0.1
    % \textbf{Self-DC} (\textit{verb}) & 24.5 & 11.6 & 40.5 \\

    % beta = 0.2
    \textit{\textbf{Self-DC}} (\textit{verb}) & 25.2 & \underline{19.5} & 52.1 \\

    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{The performance of baselines and SelfDC with the \texttt{instruct}. The baseline$^*$ means it uses demonstrations. We \textbf{bold} the highest performance and \underline{underline} the second-highest performance.}
\label{tab:append_freshqa_instruct}
\end{table}

==> tables/efficiency_ana.tex <==
\begin{table}[!t]
  \centering
  \begin{adjustbox}{max width=0.38\textwidth}
  \begin{tabular}{l|c|c|c}
    \toprule
    \textbf{Methods} & \textbf{Tims(s)} & \textbf{API(\$)} & \textbf{Retrieval} \\
    \hline
    GenRead & 739 & 0.147 & 0 \\
    RR & 468 & 0.107 & 253 \\
    IRCoT & 1,648 & 0.586 & 506 \\
    \hline
    \textit{\textbf{Self-DC}} & 982 & 0.157 & 156 \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{The efficiency analysis of different methods with \texttt{1106}. We also report the number of retrieval times in the Retrieval column.}
% \vspace{-4mm}
\label{tab:efficiency_ana}
\end{table}

==> tables/main_exp_instruct.tex <==
\begin{table}[!t]
  \centering
  \begin{adjustbox}{max width=0.48\textwidth}
  \begin{tabular}{l|ccc|ccc}
    \toprule
    \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c|}{\textbf{CuQA}} & \multicolumn{3}{c}{\textbf{FreshQA}} \\
    \cline{2-7} & EM & F1 & Acc$^\dagger$ & EM & F1 & Acc$^\dagger$  \\
    \hline
    \hline
    \multicolumn{7}{c}{\textbf{\textit{w/o retrieval}}} \\
    \hline
    \hline
    Direct & 13.0 & 5.8 & 25.3 & 19.0 & 8.2 & 38.3  \\
    CoT & 15.0 & 6.0 & 24.9 & 17.8 & 7.5 & 38.3\\
    Few-shot-CoT$^*$ & \underline{19.4} & 4.4 & \underline{31.2} & 23.3 & 13.4 & 42.0 \\
    GenRead & 16.6 & \underline{9.6} & 26.9 & 21.5 & 7.8 & 36.3  \\
    \hline
    \hline
    \multicolumn{7}{c}{\textbf{\textit{w/ retrieval}}} \\
    \hline
    \hline
    RR & 11.9 & 7.3 & 25.7 & \textbf{33.0} & 12.1 & \underline{53.8} \\
    REFEED & 6.7 & 4.5 & 26.5 & 19.2 & 10.1 & 35.7 \\
    IRCoT & 17.4 & \textbf{9.7} & 30.8 & \underline{32.8} & \textbf{21.2} & \textbf{56.5}  \\
    Self-Ask$^*$ & 7.1 & 7.4 & 24.9 & 13.8 & 16.2 & 36.7 \\
    ITER-RETGEN$^*$ & 9.9 & 6.7 & 28.5 & 14.5 & 16.0 & 43.8 \\
    \hline
    \textit{\textbf{Self-DC}} (\textit{verb}) & \textbf{21.1} & 9.4 & \textbf{35.1} & 25.2 & \underline{19.5} & 52.1 \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{The performance of baselines and \texttt{Self-DC} with the \texttt{instruct}. The baseline$^*$ means it uses demonstrations.}
% \vspace{-4mm}
\label{tab:main_exp_instruct}
\end{table}

==> templates/confidence_scores.tex <==
\begin{table}[ht]
\small
    \centering
    \colorbox{orange!8}{
    \begin{tabular}{@{}p{7.2cm}}
    Please read the question, give the answer and indicate your level of confidence. Use the following format to provide your answer and confidence level: \n\n Answer: [Your answer] \n Confidence (0-100): [Your confidence level, please only include the numerical number, e.g. 80]\% \\ 
    Note: The confidence level indicates the degree of certainty you have about your answer and is represented as a percentage. For instance, if your confidence level is 80
    \%, it means you are 80\% certain that your answer is correct and there is a 20\% chance that it may be incorrect. If you do not know the answer, simply output confidence as 0\%. \\
    \end{tabular}
    }
    \caption{Prompts to collect topics.}
    \label{tab:confidence_score}
\end{table}


